Doubly Robust Proximal Causal Learning for Continuous Treatments

Proximal causal learning is a promising framework for identifying the causal effect under the existence of unmeasured confounders. Within this framework, the doubly robust (DR) estimator was derived and has shown its effectiveness in estimation, especially when the model assumption is violated. However, the current form of the DR estimator is restricted to binary treatments, while the treatment can be continuous in many real-world applications. The primary obstacle to continuous treatments resides in the delta function present in the original DR estimator, making it infeasible in causal effect estimation and introducing a heavy computational burden in nuisance function estimation. To address these challenges, we propose a kernel-based DR estimator that can well handle continuous treatments. Equipped with its smoothness, we show that its oracle form is a consistent approximation of the influence function. Further, we propose a new approach to efficiently solve the nuisance functions. We then provide a comprehensive convergence analysis in terms of the mean square error. We demonstrate the utility of our estimator on synthetic datasets and real-world applications.

==> material.tex <==
% \subsubsection{Pseudo-outcome regression}
% In order to derive proximal double robust estimators for $\beta(a)$, we employ a novel Pseudo-outcome regression method, akin to the method elucidated by \cite{rubin2005general,kennedy2017non}. We hope to find a function $\xi(O;h,q)$ that is dependent on the observed data $O$ and the associated nuisance functions $(h, q)$. This function is devised in a manner that facilitates the construction of a "pseudo-outcome," satisfying the criterion $\mathbb E\left[\xi(O;h,q)\mid A = a\right]=\beta(a)$. Consequently, this framework culminates in the establishment of $E\left[\xi(O;h,q)\right]=\psi$, wherein
% $$
% \psi=\int\mathbb E[h_0(a,W,X)]p (a)da.
% $$
% In Theorem~\ref{theo.dr2} below, we present the efficient influence function corresponding to this parameter $\psi$, acknowledging the intrinsic uncertainty surrounding the marginal density $p(a)$.
% \begin{restatable}{theorem}{thmdrb} 
% \label{theo.dr2}
%     Under a nonparametric model, the efficient influence function for $\psi$ is $\xi(O;h,q)+\int{\left( h_0 \left( a,W,X \right) -\theta \left( a \right) \right) p\left( a \right) da}-\psi $, where
%     $$
%     \xi(O;h,q)=\left( Y-h_0(A,W,X) \right) q_0(A,Z,X)p(A) +\int{h_0\left( A,w,x \right) p\left( w,x \right) dwdx}
%     $$
% \end{restatable}

% By Theorem~\ref{theo.dr2}, this motivates us to estimate the effect curve $\beta(a)$ by estimating the nuisance functions $(h,q)$, and then regressing the estimated pseudo-outcome on treatment $A$. We can leverage flexible non-parametric regression or machine learning methods, like ridge regression, random forest, neural network, etc. to solve the final regression problem.

% \begin{equation}\label{eq.dr2}
% \hat{\mathbb{E}}_n[Y(a)]=\hat{\mathbb{E}}_n\left[\xi(O;h,q)\mid A=a\right]
% \end{equation}
% where $\hat{\mathbb{E}}_n$ represents regression with samples.
% \subsubsection{Connection Between the Two Approaches}

% It is worth noting that the two PDR estimators have double robust properties and enjoy second order rates when some regularity conditions are satisfied.

% When we utilize the kernel to approximate the indicator function, Eq.~\ref{eq.keripw} and \ref{eq.kerdr} relies on that the mean outcome to be a smooth function over the treatment space, which is also implied by previous literature \citep{kallus2018policy,cai2021deep}. When the outcome curve is non-smooth, the error curve will also be non-smooth and the estimation result of Eq.~\ref{eq.keripw} and \ref{eq.kerdr} will suffer from large approximation error. Importantly, \cite{bonvini2022fast} have similarly highlighted that the error rates they propose may adhere to a structure of "oracle + second-order terms" solely within specific smoothness regimes governing $\beta(a)$.

% In the context of Pseudo-outcome regression, the complexity of the algorithm is further heightened. Diverging from the Gateaux derivative approach, which centers its estimation efforts predominantly on the nuisance functions $(h,q)$ and allows for direct plug-in of the estimates, the Pseudo-outcome regression method necessitates an extra estimation phase for the density function $p(A)$. Moreover, it compels the subsequent step of regressing the estimated pseudo-outcome against the treatment variable $A$. These additional estimation and regression processes collectively contribute to the augmentation of algorithmic complexity.








 
